Group Scissor: Scaling Neuromorphic Computing Design to Large Neural Networks

Synapse crossbar is an elementary structure in Neuromorphic Computing Systems (NCS). However, the limited size of crossbars and heavy routing congestion impedes the NCS implementations of big neural networks. In this paper, we propose a two-step framework (namely, group scissor) to scale NCS designs to big neural networks. The first step is rank clipping, which integrates low-rank approximation into the training to reduce total crossbar area. The second step is group connection deletion, which structurally prunes connections to reduce routing congestion between crossbars. Tested on convolutional neural networks of LeNet on MNIST database and ConvNet on CIFAR-10 database, our experiments show significant reduction of crossbar area and routing area in NCS designs. Without accuracy loss, rank clipping reduces total crossbar area to 13.62\% and 51.81\% in the NCS designs of LeNet and ConvNet, respectively. Following rank clipping, group connection deletion further reduces the routing area of LeNet and ConvNet to 8.1\% and 52.06\%, respectively.

==> Area.tex <==
\vspace{-9pt}
\subsection{Area Optimization}
\label{subsec:metho:area} 
\vspace{-3pt}



==> Area_Optimization.tex <==
%\vspace{-9pt}
\subsection{Area and Routing Estimation}
\label{subsec:metho:area} 
%\vspace{-5pt}



Unlike the linear resistor, memristor behaves a non-linearity property, which means that when applying a voltage to memristor, we can't get a directly proportional current to this voltage. In a different view, It means that the resistance of memristor is not a constant. This kind of prominent inherent non-linearity property enables a set of memristors to form a cross-point structured memristor crossbar array, which can significantly achieve an ultra high density. Moreover, the minimum cell size of 4$F^{2}$ for memristor can be achieved under the state-of-the art technology\cite{xu2011design}. 
As aforementioned, the proposed memristor crossbar reduction method can significantly scale down the MBC size for every layer of neural network, so under consideration of hardware realization, it can reduce the circuit design area dramatically. We estimate the designing areas before and after crossbar reduction under the Cadence Virtuoso environment. Take \textit{Lenet}\cite{lecun1998gradient} as an example, there are four layers including two convolutional layers and two fully connected layers, both of which have different sizes. The areas estimation for different layers are shown in Fig.~\ref{Area_optimization}. In this figure, we can see that the area can be dramatically reduced after the system reduction optimization. Take the first convolutional layer as an example, the crossbar area is just 5\% of the original one. 



==> Experiment_setup.tex <==
%\vspace{-9pt}
\subsection{Experiment Setup}
\label{subsec:expri:setup} 
%\vspace{-5pt}

%%%%%%%%%%%%%%%%%%All experiments conducted in this paper are based on memristor and MBC. Related experiment parameters on memristor and MBC are summarized in Table~\ref{tab:exper_para}. We mainly implement two neural networks: $LeNet$ on MNIST and $ConvNet$ on CIFAR-10, where the detailed structure parameters are denoted in Table~\ref{tab:accu_lra_vs_clipping}.
%As described in section~\ref{subsec:metho:area} , each memristor cell occupies $4F^2$ area under the state-of-the-art technology, here $F$ is the minimum feature size. In %order to best conform to the neural network size and minimize the impact of IR-Drop and process variation, the maximum implementation crossbar size in this paper is set to %$50\times50$. 

%%%%%%%%%%%%%%%%%\input{tables/experiment_parameter}
%\input{tables/experiment_setup}


==> Low_Rank_Approximation.tex <==
%\vspace{-9pt}
\subsection{Low Rank Approximation}
\label{subsec:preli:lowrank} 
%\vspace{-5pt}

As aforementioned, there exits many hardware limitations in realizing neural network on NCS. 
In order to overcome these limitations and minimize their effect, low rank approximation is put forward in this work. \textit{Low rank approximation} is a mathematical minimization technology, which uses approximating matrices with reduced rank to approximate a given matrix. 
As demonstrated in Figure \ref{rank_clipping}, the original matrix (left one with black circles) can be approximated by two matrices (the middle one with red circles and the right one with green circles under solid boxes), both of which are much more skinny. \textit{Principal Components Analysis} (PCA) and \textit{Singular Value Decomposition} (SVD) are two commonly used low rank approximation methods. The algorithm details of PCA will be stated in section \ref{subsec:metho:pca}.

==> MBC_area_estimation.tex <==
%\vspace{-9pt}
\subsection{MBC Area Reduction}
\label{subsec:expri:MBC} 
%\vspace{-5pt}

Figure~\ref{fig:pca_rank_reduction} demonstrates the final clipping results for the two convolutional layers of $Lenet$. As we can easily see in the figure, for both two layers, the rank numbers are decreasing significantly. This is extremely important to the neuromorphic computing system design as it can largely save hardware cost and improve the system robustness and reliability. 

\begin{figure}
	\begin{center}
		\includegraphics[width=0.65\columnwidth]{figures/PCA_before_after_v2-crop.pdf}		
	    %\vspace{-6pt}
		\caption{MBC size clipping for two convolutional layers of $Lenet$. The $diamond$ and $circle$ demonstrate the first and second convolutional layers, respectively. The dark green and the light green diamond show the rank number before and after the clipping, respectively. And it is the same with the dark red and light red circles.} 
		\label{fig:pca_rank_reduction}
		\vspace{-15pt}
	\end{center}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[width=1\columnwidth]{figures/Area.pdf}		
		%\vspace{-6pt}
		\caption{} 
		\label{fig:Area_optimization}
		\vspace{-15pt}
	\end{center}
\end{figure}

==> Memristor_and_Crossbar_Basics.tex <==
%\vspace{-9pt}
\subsection{NCS for big neural networks}
\label{subsec:preli:memristor} 
%\vspace{-5pt}

%Brain-inspired \textit{Neuromorphic Computing System} (NCS) is one of the most promising architectures for hardware implementation of neural networks. 
%Memristor, as an extremely important component in NCS and behaving a non-volatile resistive property, mimics the biological function of synapse in neural networks. 
Fig.~\ref{NN_xbar}(a) demonstrates an implementation of a convolutional layer in neural networks using \textit{Memristor-based Crossbars} (MBC), where memristors (synapses) in each column encode the weights of one filter \cite{linghao2017pipelayer}\cite{?asp-dac}. The implementation of a fully-connected layer is similar, but each column realizes the connections to one output neuron~\cite{?}. As aforementioned, the sizes of crossbar are limited, which demands the interconnection of crossbars to implement big neural networks. 
Fig.~\ref{NN_xbar}(b) depicts a circuit-level implementation of a big layer by tiling and interconnecting MBC~\cite{?}. 
As the scale of modern neural networks grows, the high crossbar occupation and heavy routing congestion become critical issues and seriously obstruct the scalability of the design to big neural networks~\cite{?}. We propose the \textit{Group Scissor} framework to improve the scalability of neuromorphic computing design.





%Therefore, there is a big gap between the NCS and big neural network implementations. Moreover, employing many small size crossbars to implement big neural network will inevitably bring in much more routing connections among different crossbars.


 \begin{figure}[t] 
	\begin{center}
		\includegraphics[width=1\columnwidth]{figures/NN_xbar-crop.pdf}		
		\vspace{-15pt}
		\caption{NCS design for a neural network with convolutional layer and fully connected layer.} 
		\label{NN_xbar}
		\vspace{-15pt}
	\end{center}
\end{figure}

==> PCA.tex <==
%\vspace{-9pt}
\subsection{Principal Components Analysis}
\label{subsec:metho:pca} 
%\vspace{-5pt}

As aforementioned, there exits many hardware limitations in realizing neural network on NCS. 
In order to overcome these limitations and minimize their effect, low rank approximation is put forward in this work. \textit{Low rank approximation} is a mathematical minimization technology, which uses approximating matrices with reduced rank to approximate a given matrix. 
As demonstrated in Figure \ref{rank_clipping}, the original matrix (left one with black circles) can be approximated by two matrices (the middle one with red circles and the right one with green circles under solid boxes), both of which are much more skinny. \textit{Principal Components Analysis} (PCA) and \textit{Singular Value Decomposition} (SVD) are two commonly used low rank approximation methods. The algorithm details of PCA will be stated in section \ref{subsec:metho:pca}.

In this paper, Principal Components Analysis (PCA) method is employed to reduce the large sizes of Neural Network weight matrix to small sizes which can be actually implemented in MBC. The essence operation of PCA is to make a linear projection for data from a high dimensional space ($\textbf{x}_{i}\in\mathbb{R}^d$) to a lower dimensional subspace ($\textbf{y}_{i}\in\mathbb{R}^m$, $m\ll d$) \cite{jolliffe2002principal}. The step-by-step calculations of this algorithm are depicted elaborately in Algorithm 1.  
		
\begin{algorithm}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\caption{Principal Components Analysis (PCA)}
\Input{$N \times d$ matrix $\textbf{W}$}
Calculate mean of dataset $\textbf{w}_{i} \in \textbf{W}$:  $\mu=\frac{1}{N}\sum_{i=1}^{N}\textbf{w}_{i}$;\\
Centralized the data: replace each $\textbf{w}_{i}$ with $\textbf{w}_{i}-\mu$;\\
Calculate the $d \times d$ covariance matrix: $\textbf{C}=\dfrac{1}{N-1}\textbf{W}^{T}\textbf{W}$;\\
Calculate the eigenvectors $\textbf{v}_{i}$ and eigenvalues $\textbf{$\lambda$}$ of covariance matrix $\textbf{C}$: $\textbf{C}\textbf{v}_{i}=\lambda_{i}\textbf{v}_{i}$;\\
Project the data: $N\times m$ matrix $\widetilde{\textbf{W}}=\textbf{W}\textbf{V}$, where $\textbf{V}=[{\textbf{v}_{1}},...{\textbf{v}_{m}}]$ is a $d\times m$ matrix where each ${\textbf{v}_{i}}$ are eigenvectors to the corresponding largest $m$ eigenvalues of $\textbf{C}$;\\
\Output{$N \times m$ matrix $\widetilde{\textbf{W}}$, $m\ll d$}
%The eigenvectors with the highest $m$ eigenvalues are the principle components of the data.
\end{algorithm}

The above PCA algorithm have formulated the equation between input matrix $\textbf{W}$ and output matrix $\widetilde{\textbf{W}}$. Derived from this equation and under the prerequisite condition that $\textbf{V}\textbf{V}^{T}=\textbf{I}$, we can easily get another equation $\textbf{W}=\widetilde{\textbf{W}}\textbf{V}^{T}$. As aforementioned, $\widetilde{\textbf{W}}$ is the linear projection in a lower subspace of $\textbf{W}$ from a higher dimensional space. Therefore, $N \times d$ matrix $\textbf{W}$ can be substituted by two smaller matrices $\widetilde{\textbf{W}}$($N \times m$) and $\textbf{V}$($d \times m$). This process is usually called \textit{matrix factorization}.


==> Routing_area_estimation.tex <==
%\vspace{-9pt}
\subsection{Routing Area Estimation}
\label{subsec:expri:rout} 
%\vspace{-5pt}

==> Total_area_reduction.tex <==
%\vspace{-9pt}
\subsection{Total Area Reduction}
\label{subsec:expri:total_area} 
%\vspace{-5pt}

==> tables/experiment_setup.tex <==
\begin{table}[t]
	\caption{Neural network and dataset}
	\label{tab:fc:setup}
	%\vspace{-6pt}
	\centering
	\footnotesize
		\def\arraystretch{1}\tabcolsep 15pt
		%\def\thefootnote{a}\footnotesize
		%\begin{tabular}{l@{~}l@{~~~}l}
		\begin{tabular}{c c c c}
			\toprule [0.1 em]
			\toprule [0.1 em]	
			\parbox[c]{1mm}{} & Network 1 & Network 2\\
			\midrule [0.07 em]
			Dataset   & MNIST  & CIFAR-10\\
			Input      & 28$\times$28              & 32$\times$32\\
			conv1     & 20$\times$5$\times$5\textsuperscript{\textsection}      & 32$\times$5$\times$5\\   
			conv2     & 50$\times$5$\times$5      & 32$\times$5$\times$5\\ 
		    conv3     & $-$                       & 64$\times$5$\times$5\\   
			fc1       & 800$\times$500               & 1024$\times$10\\
			fc2       & 500$\times$10                & $-$\\
			\bottomrule [0.1 em]
			\bottomrule [0.1 em]
		\end{tabular}
		%\footnotetext[1]{\scriptsize $\xi$ 20$\times$5$\times$5 means 20 kernels with each kernel size 5$\times$5.}
		%\footnotetext{\textsuperscript{\textsection}20$\times$5$\times$5 means 20 kernels with each kernel size 5$\times$5.}
		
		%\vspace{3pt}
		\textsuperscript{\textsection}20$\times$5$\times$5 means 20 filters with each filter size 5$\times$5.
	\vspace{-12pt}
\end{table}



==> tables/iclr_speedups.tex <==
\begin{table*}
  \caption{ The speedup benefit from similarity regularization in state-of-the-art work~\cite{Cheng_arxiv_2015} (\textit{AlexNet}).}
  \label{tab:iclr_speedups}
  \centering
  %\resizebox{\textwidth}{!}{
  	\begin{tabular}{cccc|rrrrrr}
  		\toprule [0.12 em]
  		\textit{AlexNet} & Regularization &  $\frac{e_M}{e_0}$ & Top-1 error & & conv1 & conv2 & conv3 & conv4 & conv5   \\
  		\midrule [0.12 em]
  		
  		\multirow{3}{*}{1} & \multirow{3}{*}{None}\textsuperscript{$\dagger$}  & \multirow{3}{*}{20\%} & \multirow{3}{*}{43.21\%} & rank \textsuperscript{$\ddagger$}
  		& 27 & 88 & 184 & 201 & 146  \\
  		&&&& speedup $\times$ &  1.24 & 1.47  & 1.58 & 1.21 & 1.15\\
  		&&&& theo.\textsuperscript{$\ast$} $\times$ &  2.81 & 2.63  & 1.79& 1.72 & 1.63 \\
  		
  		% & SVD\textsuperscript{$\dagger$} & -- & \% &  &  & & & & \\
  		% & k-means\textsuperscript{$\dagger$} & -- & \% &  &  & & & & \\
  		 
  		 \cmidrule{1-10}
  		 
  		 \multirow{3}{*}{2} & \multirow{3}{*}{$\ell_2$-norm force} &   \multirow{3}{*}{15\%} & \multirow{3}{*}{43.25\%} & rank
  		 & 33 & 100 & 124 & 106 & 129  \\
  		 &&&& speedup $\times$ &  1.23 & 1.47  & 2.16 & 2.03 & 1.33 \\
  		 &&&& theo. $\times$ &  2.30 & 2.31  & 2.65 & 3.26 & 1.85 \\
  		 
  		 % & SVD\textsuperscript{$\dagger$} & -- & 43.20\% & &  &  & & &  \\
  		 % & k-means\textsuperscript{$\dagger$} & -- & 44.80\% &  &  & & & & \\
  		 
  		 
  		 \cmidrule{1-10}
  		 \multirow{3}{*}{3} & \multirow{3}{*}{$\ell_1$-norm force} &  \multirow{3}{*}{15\%} & \multirow{3}{*}{43.02\%} & rank
  		 & 33 & 100 & 130 & 91 & 128  \\
  		 &&&& speedup $\times$ &  1.23 & 1.47 & 1.65 & 2.06 & 1.34 \\
  		 &&&& theo. $\times$ & 2.30 &  2.31 & 2.53  & 3.80 & 1.86  \\
  		 
  		 \cmidrule[0.12 em]{1-10} 
  		 \multirow{3}{*}{4} & \multirow{3}{*}{$\ell_2$-norm force} & \multirow{3}{*}{20\%} & \multirow{3}{*}{44.10\%} & rank
  		 & 29 & 83 & 95 & 74 & 105  \\
  		 &&&& speedup $\times$ &  1.25 & 1.51  & 2.22& 2.10 & 1.58 \\
  		 &&&& theo. $\times$ &  2.62 & 2.79  & 3.46 & 4.67 & 2.27 \\
  		
  		\bottomrule [0.12 em]
  		\multicolumn{10}{l}{\textsuperscript{$\dagger$} The baseline. \textsuperscript{$\ddagger$} The full rank is 96, 256, 384, 384 and 256, respectively. \textsuperscript{$\ast$} Theoretical speedup.}
  	\end{tabular}
  %}
\end{table*} 
